NVCell: Standard Cell Layout in Advanced Technology Nodes with Reinforcement Learning

High quality standard cell layout automation in advanced technology nodes is still challenging in the industry today because of complex design rules. In this paper we introduce an automatic standard cell layout generator called NVCell that can generate layouts with equal or smaller area for over 90% of single row cells in an industry standard cell library on an advanced technology node. NVCell leverages reinforcement learning (RL) to fix design rule violations during routing and to generate efficient placements.

==> placement.tex <==
\section{Placement}
Given a set of PMOS and NMOS devices, the goal of placement is to place them on the PMOS row and NMOS row of the cell layout while satisfying technology constraints. The technology constraints \textbf{NVCell} honors include the diffusion sharing rule, the fin number matching rule and gate matching rule. The diffusion sharing rule dictates if two adjacent devices do not share diffusion, there must exist at least $K_s$ dummy polys separating them. The fin number matching rule dictates that if two adjacent devices have different number of fins, there must exist at least $K_f$ dummy polys separating them.  The gate matching rule dictates that if a PMOS device and a NMOS device share the same poly gate, they must have the same gate signal. 

For our placer implementation, we prefer a technique that can adapt to custom layout constraints and is easy to implement. Therefore we choose to use a simulated annealing algorithm. Previous placers often separate placement into two steps: pairing and ordering. The pairing step pairs up each PMOS device with a NMOS device to form device pairs. Paired devices should satisfy the gate matching rule. The ordering step generates placement order of device pairs. And the final placement can be inferred from placement order and pairs. These two steps are interdependent, so solving one after the other is sub-optimal. Therefore we design an simulated annealing based algorithm that does both pairing and ordering simultaneously. 

\textbf{Placement Representation} Given a total number of placement pairs $N\geq max(N_{P}, N_{N})$, where $N_{P}$ and $N_{N}$ are number of PMOS and NMOS devices, respectively. The placement representation is given by the PMOS placement order $\{I^P_1,...,I^P_{N}\}$ where $I^P_x$ is a PMOS device index in the range of $[1,...,N_P]$, the NMOS placement order $\{I^N_1, ..., I^N_{N}\}$ where $I^N_x$ is a NMOS device index in the range of $[1,...,N_N]$, and device flip flags $\{R^P_1,...R^P_{N_P}\}$ and $\{R^N_1,...,R^N_{N_N}\}$ indicating whether source and drain diffusions of the device indexed by $x$ should switch or not.   If $N>N_P$, $N-N_P$ number of $I^P_x$ will have \textit{NULL} value. If $N>N_N$, $N-N_N$ number of $I^N_x$ will have \textit{NULL} value. This representation uniquely specifies the placement of all the devices within a cell. 

In addition to device placement, cell pin locations should also be specified during placement. We define pin locations as $\{P_1, ..., P_N\}$, where $P_x$ is the index of pin placed near the $x$th placement pair. Usually there are less pins $M$ than placement pairs $N$, therefore there are $N-M$ \textit{NULL} values in pin locations.  



\begin{comment}


The detail algorithm is given in Algorithm \ref{alg:placement}. 

\begin{algorithm}[h!]
\caption{Placement Generation From Placement Representation}
\label{alg:placement}
\begin{algorithmic}

\Require placement representation $I^P_1,...,I^P_{N}$, $I^N_1, ..., I^N_{N}$, $R^P_1,...R^P_{N_P}$ and $R^N_1,...,R^N_{N_N}$
 
\Ensure Placement location of each device $x^P_1,..., x^P_{N_P$ and $x^N_1,..., x^N_{N_N$
 

\State {$x$ \gets $0$}
 
\For {$k \gets 1$ \textbf{to} $N$ } 

\If {$I^P_k$ is not \textbf{NULL}} 

\State {$x^P_{I^P_k}$ \gets $x$}

\EndIf

\If {$I^N_k$ is not \textbf{NULL}} 

\State {$x^N_{I^N_K}$ \gets $x$}

\EndIf 

\State {$x$ \gets $x+1$}
 
\If {devices ($I^P_k$, $I^P_{k+1}$) \textbf{or} ($I^N_k$, $I^N_{k+1}$) have different fin numbers}
 
\State {$x$ \gets $x + K_f$ }
 
\ElsIf {devices ($I^P_k$, $I^P_{k+1}$) \textbf{or} ($I^N_k$, $I^N_{k+1}$) do not share diffusion}
 
\State {$x$ \gets $x + K_s$}
 
\EndIf
 
\EndFor
 
\end{algorithmic}

\end{algorithm}
\end{comment}



\textbf{Simulated Annealing} Simulated annealing makes \textit{moves} on the placement representation to optimize the scoring function. These \textit{moves} can be categorized either by the types of moves and by the targeted devices of the moves. The \textit{Flip} changes all targeted devices flip flag. The \textit{Swap} swaps targeted devices. The \textit{Move} moves targeted devices to a specific location. The target devices can be either a consecutive of PMOS devices, or a consecutive NMOS devices, or a consecutive PMOS/NMOS device pairs, or pins. 

The scoring function is a weighted sum of minimum width of the cell, estimated congestion, and violation counts. The minimum width of cell is determined after placement of the representation, which traverse the device placement order $\{I^P_1,...,I^P_{N}\}$ and $\{I^N_1, ..., I^N_{N}\}$ from left to right to compute the location of each device based on technology constraints. The pins will be placed near the placement pairs they are associated with. The estimated congestion is based on the maximum crossing of all nets over a vertical edge. The violation counts are the number of device pairs violating the gate matching rule.



\begin{comment}
The moves are shown in Table \ref{table:sa}. 
\begin{table}
  \caption{Simulated Annealing Move Types}
  \label{table:sa}
  \centering
  \begin{tabular}{llll}
    \toprule
    Categories     & \textit{Flip} & \textit{Swap} & \textit{Move}\\
    \midrule
    PMOS & 1      & 2 & 3     \\
    NMOS     & 4 & 5 &6 \\
    PMOS/NMOS     & 7 & 8 & 9 \\
    Pin & &10 & \\
    \bottomrule
  \end{tabular}
\end{table}
\end{comment}
The simulated annealing algorithm is implemented based on the modified Lam annealing schedule \cite{adaptiveSA} that requires no hyper-parameter tuning. 



==> router.tex <==
\section{Routing}
\textbf{NVCell} router has two steps: a genetic algorithm-based routing step and a RL-based DRC fixing step. In this section we first describe RL-based DRC fixing step, then the genetic algorithm for the routing step. 

\subsection{RL-based DRC Fixing} 
We focus on fixing M1 DRC errors in the DRC fixing step. M1 is the lowest routing metal layer with most difficult DRC issues. Other DRC errors can be easily pruned out during maze routing. M1 DRC errors are caused by constraints for cut metal locations. The Stick program determines the cut metal locations based on the M1 routes. Therefore changing M1 routes modifies cut metal locations, which in turn change the M1 DRCs. The RL \textit{game} is then to incrementally change the M1 route in order to reduce M1 DRCs.  %as long as incremental change to the routes can modify those DRCs. 
%In this \textit{game}, 

\textbf{Observation space}: $obs$ is a Box tensor $[3,H^{M1},W^{M1}]$. $H^{M1}$ and $W^{M1}$ are the M1 grid dimension. $obs[0,:,:]$ represents the M1 routes. $obs[1,:,:]$ represents the routing mask based on some basic routing rules. $obs[2,:,:]$ represents the DRC information, it records the locations of DRC marks reported by the Stick DRC checker. 

\textbf{Action space}: $act$ is a categorical tensor $[H^{M1}\times W^{M1}]$. It represents the probability of whether any of the M1 grid $[H^{M1},  W^{M1}]$ should be routed. 

\textbf{Reward}: There are two types of rewards given by the environment. $r_s$ is a negative reward given at each step. This reward pushes the agent to finish the \textit{game} as soon as possible. %$r_n$ is a negative reward given when an illegal routing action is created. 
$r_d$ is a reward associated with DRC improvement, $r_d = R_d \times \Delta DRC$, where $R_d$ is a coefficient and $\Delta DRC$ is the reduction of number of DRC markers reported by Stick DRC checker. This reward drives the agent to reduce DRCs as much as possible. 

\textbf{Done condition}: in two conditions the environment will tell agent it's done. First when an illegal action is given to the agent. Second when DRC is zero, i.e. the DRC layer $obs[2,:,:] = 0$. 



\begin{figure*}[h]
  \centering
  \includegraphics[trim={0in 2.5in 0in 2.5in},clip, width=\textwidth]{figs/model_new.pdf}
  \caption{DRC RL Model Architecture}\label{fig:model}

\end{figure*}

We use Proximal Policy Optimization (PPO) \cite{PPOSchulman} algorithm for our DRC fixing step. PPO is a policy gradient based RL algorithm. It has been shown to achieve state of the art results on many discrete and continuous tasks. The key advantages of PPO algorithm are ease of implementation, simpler sample complexity, and ease of tuning. 

To build a RL model for PPO, we need to consider two requirements: first it should be invariant to the number of nets, and second it should be invariant to the cell width, i.e. $W^{M1}$. Note that $H^{M1}$ is a constant given a standard cell library. 

The observation space is actually independent of number of nets, therefore the first requirement is satisfied. The second requirement, however, is not satisfied by default since the observation space and the action space are both dependent on $W^{M1}$. To eliminate this dependency, we designed the network as shown in Figure~\ref{fig:model}.


The observation $obs$ is first fed to four convolution layers. Each convolution layer uses VALID padding scheme to produce output activation with the same height and width as the input. The output of the last convolution layer is the state embedding, which has a shape of $[512,H^{M1},W^{M1}]$. Then this state embedding is fed to both the value and the policy network. The policy network has three fully connected layers with channel size (64,64,1). We feed each pixel of the state embedding image to these fully connected layers. Since the channel dimension of each pixel on the state embedding image is fixed, which is 512, the parameters of those fully connected layers are not dependent on the size of the image. Then the outputs of the policy networks for all the $H^{M1}\times W^{M1}$ pixels are collected together, masked by the action mask from the observation, and fed to a softmax layer to produce the final action policy vector. 

To produce state value, the embeddings of all the pixels are avg-pooled together to form a 512 wide vector. Then it is fed to the value network composed of three fully connected layers with channel size (64,64,1). The output of this value network is the state value.  Again the value network is not dependent on the size of the image. 

\subsection{Genetic Algorithm based Routing}
Although DRC RL agent can reduce the number of DRCs of a given routed cell by adding extra M1, it can not rip up and reroute existing route. Therefore we need a high level exploration of different routes in order to find routes whose DRCs can be fully fixed by the DRC RL agent. We choose to leverage genetic algorithm for this task. 
Because there are multiple routing candidates in each genetic generation, it is possible that more than one candidate can be made DRC free. Therefore this flow might generate multiple routing solutions in addition to DRC optimization, which is an extra advantage.  

We adopt the routing segments based genetic encoding strategy as used in channel routing \cite{GALienig} and \cite{GAGockel}.% Routing segments, i.e. partial routing structures connecting terminals or Steiner points, are recorded. 
 The benefit of using routing segments as genetic representation is in that it ensures that good "routing islands" in the routing structure are preserved during genetic operations such as crossover and mutation. We extend this strategy with our random maze router and support for Stick environment. The complete routing flow is shown in Algorithm \ref{alg:routing}.

\begin{algorithm}[h!]
\caption{Genetic Algorithm-based Routing Flow}
\label{alg:routing}
\begin{algorithmic}

  \Require nets $\mathbb{N}$, net terminals $\mathbb{T}_n$, generations $G$, population $K$
  %horizontal cut probability $Prob_h$, crossover probability $Prob_c$, mutation probability $Prob_m$,
 
 \Ensure DRC free routing solution $\mathbb{R}$

 \State create the terminal pair set $\mathbb{P}$
 

 \State initialize routing solutions $\{\mathbb{R}_1,...,\mathbb{R}_k\}$ for the first generation with random routing order
 
 
 \For {$g \gets 1$ \textbf{to} $G$ }
 \For {$i \gets 1$ \textbf{to} $K$ }
 \State select $\mathbb{R}_{dad}$ and $\mathbb{R}_{mom}$ from $\{\mathbb{R}_1,...,\mathbb{R}_k\}$
 
 \State $\mathbb{R}' \gets crossover(\mathbb{R}_{dad}, \mathbb{R}_{mom}) $
 \State $\mathbb{R'} \gets mutate(\mathbb{R'})$
 \State  $\mathbb{R'}_i \gets$ Maze route unrouted pairs with random order 
 \State run RL DRC fixer on route $\mathbb{R'}_i$
 \State $DRC(\mathbb{R'}_i) \gets $ remaining DRCs
 \If {$DRC(\mathbb{R'}_i)==0$}
 \State return $\mathbb{R'}_i$
 \EndIf
 \EndFor
 \State $\{\mathbb{R}_1,...,\mathbb{R}_k\}$ $\gets$ Top $K$ fitness from $\{\mathbb{R'}_1,...,\mathbb{R'}_k, \mathbb{R}_1,...,\mathbb{R}_k\}$
 \EndFor
 
\end{algorithmic}

\end{algorithm}
\textbf{Genetic Representation}: The genetic representation of a routing solution, i.e. chromosome, is a set of routing segment $\mathbb{R} = \{r(p), \forall p \in \mathbb{P}\}$. $r(p)$ represents the routing segments for each terminal pair $p$ in a set of terminal pairs $\mathbb{P}$. These routing segments are created with a maze router based on Lee algorithm. 

%\subsubsection{Fitness}
\textbf{Fitness}: The fitness $f(\mathbb{R}_i)$ of each individual $\mathbb{R}_i$ in a generation is evaluated based on two metrics: the number of unrouted terminal pairs and the number of DRCs. Other metrics can be also added into fitness function, such as total wiring cost or DFM metrics. 

\textbf{Crossover}: The crossover of two genes work as follows: First it picks a cut point in the cell image. The cut can be either vertical or horizontal. For vertical cut, the crossover operator takes all the $r_{mom}(p)$ that are completely on the left hand side of the vertical cut, and all the $r_{dad}(p)$ that are completely on the right hand side of the cut. The crossover operator also generates another descendant with right side routes from $\mathbb{R}_{mom}$ and left side routes from $\mathbb{R}_{dad}$. Horizontal cut is processed similarly. 

%\subsubsection{Mutation }
\textbf{Mutation}: For each descendant generated by crossover operator, the mutation operator randomly selects a region in the cell image and remove any $r(p)$ in the descendant that touches this region. After mutation, the remaining open terminal pairs will be routed with the maze router using a random terminal pair order. 

==> sticks.tex <==
\section{Stick Environment} \label{stick_sec}

Stick diagrams have been used for decades to sketch out the rough layout of a circuit on a whiteboard or napkin before proceeding to draw the real thing \cite{uyemura2002introduction}.  They allow a designer to rapidly prototype various designs without going through the time-consuming process of creating actual layout.  Although stick diagrams were extremely helpful in the past for planning device placement, with the advent of fully gridded layout, it is now possible for a simple stick diagram to contain all the information necessary to create real DRC clean layout.  We built a GUI driven tool called Sticks that does just that.

Since all base layer shapes and metal shapes within a standard cell are now restricted to a small set of allowable locations, we assembled a library of layout subcells which included every possible shape that could be drawn while adhering to our library template and DRC rules.  In older process technologies without fully gridded routing, the size of this library would have been impracticably large.  Every existing standard cell in our library can be built by simply composing these subcells in various ways.  

By abstracting away as much layout information as possible, Sticks reduces the set of mask layers that need to be drawn from 30-40 to 5.  It also abstracts away details the designer has no control over such as wire width and pitch, and only allows shapes to be drawn on track in legal locations.  Sticks also automatically determines where to cut certain base layers, if a legal solution can be found, abstracting those layers away almost entirely.  Vias, pins, and text labels are also inferred automatically.  When routing the design, online DRC checking provides instant feedback on what is legal or illegal.

The layout can be exported as a Skill script or streamed directly to a Virtuoso session.  Sticks can also be driven via automation tools, and provides an API for importing layout and checking DRCs.

